Tuning of multivariable model predictive controllersthrough expert bandit feedback

For certain industrial control applications an explicit function capturing the nontrivial trade-off between competing objectives in closed loop performance is not available. In such scenarios it is common practice to use the human innate ability to implicitly learn such a relationship and manually tune the corresponding controller to achieve the desirable closed loop performance. This approach has its deficiencies because of individual variations due to experience levels and preferences in the absence of an explicit calibration metric. Moreover, as the complexity of the underlying system and/or the controller increase, in the effort to achieve better performance, so does the tuning time and the associated tuning cost. To reduce the overall tuning cost, a tuning framework is proposed herein, whereby a supervised machine learning is used to extract the human-learned cost function and an optimization algorithm that can efficiently deal with a large number of variables, is used for optimizing the extracted cost function. Given the interest in the implementation across many industrial domains and the associated high degree of freedom present in the corresponding tuning process, a Model Predictive Controller applied to air path control in a diesel engine is tuned for the purpose of demonstrating the potential of the framework.

==> Archive 2/math_notation.tex <==
% Some math operators
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator*{\arginf}{\arg\!\inf}
\DeclareMathOperator*{\argmin}{\arg\!\min}

%% "Standard"

\newcommand{\RealSet}{\mathbb{R}} % Set of real numbers
\newcommand{\IntegerSet}{\mathbb{Z}} % Set of integer numbers
\newcommand{\NaturalSet}{\mathbb{N}} % Set of natural numbers
\newcommand{\TimeSet}{\mathcal{T}}% Time set
\newcommand{\IntervalSet}{\mathcal{I}} % Interval set
\newcommand{\DummySet}{\mathbb{D}} % Dummy set
\newcommand{\DomainSet}{\mathcal{D}} % Domain set

\newcommand{\System}{\Sigma} % System
\newcommand{\State}{x} % System state
\newcommand{\Input}{u} % System input
\newcommand{\Reference}{r} % System reference
\newcommand{\Output}{y} % System output

\newcommand{\SamplingTime}{T_s}% Sampling time

\newcommand{\AMatrix}{A} % Matrix A
\newcommand{\BMatrix}{B} % Matrix B
\newcommand{\CMatrix}{C} % Matrix C
\newcommand{\DMatrix}{D} % Matrix D

\newcommand{\StateMap}{f} % State mapping
\newcommand{\OutputMap}{h} % Output mapping
\newcommand{\TransitionMap}{\phi} % Transition mapping

\newcommand{\StateSet}{\mathcal{X}} % State Set
\newcommand{\OutputSet}{\mathcal{Y}} % Output Set
\newcommand{\InputSet}{\mathcal{U}} % Input Set

\newcommand{\StateDimension}{n} % State dimension
\newcommand{\OutputDimension}{p} % Output dimension
\newcommand{\InputDimension}{m} % Input dimension
\newcommand{\ReferenceDimension}{l} % Reference dimension

%% Theorems

\newtheorem{theorem}{Theorem}
\newtheorem{assumption}{Assumption}
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}

%% Custom

%__system_parameter
\newcommand{\SystemParameter}{\theta} % System parameter
\newcommand{\SystemParameterSet}{\Theta} % System parameter set
\newcommand{\SystemParameterSetDiscretized}{\Theta^\sharp} % System parameter set
\newcommand{\SystemParameterDimension}{b} % System parameter dimension
\newcommand{\SystemParameterPerturbed}{\tilde{\SystemParameter}} % System parameter perturbed
\newcommand{\SystemParameterSteadyState}{\SystemParameter_{ss}} % System parameter at steady state
\newcommand{\SystemParameterEquilibrium}{\SystemParameter_{e}} % System parameter at the equilibrium

%__perturbed--system_elemets
\newcommand{\StatePerturbed}{\tilde{\State}}
\newcommand{\InputPerturbed}{\tilde{\Input}}
\newcommand{\OutputPerturbed}{\tilde{\Output}}


%__steady--system_elements
\newcommand{\StateSteadyState}{\State_{r}} % "Steady-state" state
\newcommand{\OutputSteadyState}{\Output_{r}} % "Steady-state" output
\newcommand{\InputSteadyState}{\Input_{r}} % "Steady-state" input

%__eco_optimal_steady--system_elements
\newcommand{\StateEcoSteadyState}{\State_{r}^\star} % Economically optimal "Steady-state" state
\newcommand{\OutputEcoSteadyState}{\Output_{r}^\star} % Economically optimal "Steady-state" output
\newcommand{\InputEcoSteadyState}{\Input_{r}^\star} % Economically optimal "Steady-state" input

%__quilibrium_elements
\newcommand{\EquilibriumState}{\State_{e}} % Equilibrium state
\newcommand{\EquilibriumOutput}{\Output_{e}} % Equilibrium output
\newcommand{\EquilibriumInput}{\Input_{e}} % Equilibrium input

%__mvem--parameter
\newcommand{\MVEMSetpoint}{\theta} % Setpoint theta
\newcommand{{\MVEMSetpointSet}}{\Theta} % Setpoint theta set

%__mvem--engine_variables:
\newcommand{\PressureIn}{p_{in}} % Pressure in the intake manifold
\newcommand{\DensityIn}{\rho_{in}} % Density in the intake manifold
\newcommand{\BurntGasIn}{F_{in}} % Burnt Gas Proportion in the intake manifold
\newcommand{\PressureEx}{p_{ex}} % Pressure in the exhaust manifold
\newcommand{\DensityEx}{\rho_{ex}} % Density in the exhaust manifold
\newcommand{\BurntGasEx}{F_{ex}} % Burnt Gas Proportion in the exhaust manifold
\newcommand{\PressurePreThrottle}{p_{pth}} % Pressure in the pre-throttle manifold
\newcommand{\TemperatureCombustion}{T_{com}} % Temperature of the combustion products
\newcommand{\TemperatureEGR}{T_{EGR}} % Temperature at the outlet of the EGR cooler
\newcommand{\EGRRate}{F_{EGR}} % EGR rate
\newcommand{\PumpLoss}{p_{loss}} % Pumping loss
\newcommand{\InputThrottle}{\Input_{thr}} % Throttle position
\newcommand{\InputEGR}{\Input_{EGR}} % EGR valve position
\newcommand{\InputVGT}{\Input_{VGT}} % Setting of the VGT
\newcommand{\RotationalSpeed}{\Omega} % Turbocharger rotational speed
\newcommand{\EngineSpeed}{w} % Engine speed
\newcommand{\VolumetricFuel}{w_{fuel}} % Volumetric flow-rate

%__mpc--matrices:
\newcommand{\MPCMatrixQ}{Q} % Matrix Q
\newcommand{\MPCMatrixR}{R} % Matrix R
\newcommand{\MPCMatrixP}{P} % Matrix P

%__mpc--horizon:
\newcommand{\MPCHorizon}{N} % MPC horizon

%__mpc--cost-function:
\newcommand{\MPCCost}{J}

